The ACAC_D Model for Mutable Activity Control and Chain of Dependencies in Smart and Collaborative Systems

With the integration of connected devices, artificial intelligence, and heterogeneous networks in IoT-driven cyber-physical systems, our society is evolving as a smart, automated, and connected community. In such dynamic and distributed environments, various operations are carried out considering different contextual factors to support the automation of collaborative devices and systems. These devices often perform long-lived operations or tasks (referred to as activities) to fulfill larger goals in the collaborative environment. These activities are usually mutable (change states) and interdependent. They can influence the execution of other activities in the ecosystem, requiring active and real-time monitoring of the entire connected environment. Recently, a vision for activity-centric access control(ACAC) was proposed to enable security modeling and enforcement from the perspective and abstraction of interdependent activities. The proposed ACAC incorporates four decision parameters: Authorizations(A), oBligations(B), Conditions(C), and activity Dependencies(D) for an object agnostic access control in smart systems. In this paper, we take a step further towards maturing ACAC by focusing on activity dependencies(D) and developing a family of formal mathematically grounded models, referred to as ACAC_D. These formal models consider the real-time mutability of activities in resolving active dependencies among various activities in the ecosystem. Activity dependencies can form a chain where it is possible to have dependencies of dependencies. In ACAC, we also consider the chain of dependencies while handling the mutability of an activity. We highlight the challenges while dealing with chain of dependencies, and provide solutions to resolve these challenges. We also present a proof of concept implementation of with performance analysis for a smart farming use case.

==> Algorithms/Algorithm1_conflict_detection.tex <==
\begin{algorithm*}[!htb]
\caption{Detecting Conflicting Desired States of Dependent Activities}
\label{alg:algorith}
\begin{algorithmic}
\State \textbf{\textbf{CHECK-DETECT-CHAIN-OF-DEPENDENCIES($da, da\_current\_st, da\_desired\_st$)}}:
\end{algorithmic}

\begin{algorithmic}[1]
\State DETECT-CONFLICTING-DESIRED-STATE($da, da\_desired\_st$)
\State $DoDA = getDoDA(da,da\_current\_st,da\_desired\_st)$
\State \textbf{if} ($DoDA \neq \emptyset$)
\State \textbf{then}
\For{(each $doda$ \in $DoDA$)}
\State \textbf{CHECK-CHAIN-OF-DEPENDENCIES}($doda, getCurrentSt(doda)$,
\State$getDesiredDoDASt(da,da\_current\_st,da\_desired\_st,doda)$)\\
\end{algorithmic}
\begin{algorithmic}
\State \textbf{\textbf{DETECT-CONFLICTING-DESIRED-STATE}}($da, da\_desired\_st$):
\end{algorithmic}
\begin{algorithmic}[1]
\State \textbf{if} ($assignedDesiredSt(da)$ == \emptyset)    
%\State $getCurrentSt(da) = da\_desired\_st$
    \State \textbf{then} $assignedDesiredSt(da) = da\_desired\_st$\\
    $hasConflictingDesiredSt(da) = FALSE$
    \State \textbf{else if} $da\_desired\_st \neq assignedDesiredSt(da)$
\State \textbf{then} $hasConflictingDesiredSt(da) = TRUE$
\State \textbf{else} $hasConflictingDesiredSt(da) = FALSE$
\State \textbf{end if}
\end{algorithmic}
%\end{algorithmic}
\end{algorithm*}

==> Sections/Chain_of_dependencies.tex <==
\begin{figure}[!htb]
    \centering
\includegraphics[width=.5\columnwidth]{Figures/multiple_dependency_path.png}
    \centering
    \caption{Chain of Dependencies with Multiple Dependency Paths.}
    \label{fig-multiple_dependency_path}
     %\vspace{-3mm}
\end{figure}
\vspace{-3mm}
\input{Sections/Challenges_chain_of_dependencies}


==> Sections/Formal_updated.tex <==
\section{Towards formal ACAC Policy Models}
\subsection{$\mathrm{ACAC_{ABCD}}$ Core Models}
The four components \cite{mawla2022bluesky}, Authorizations(A), Obligations(B), Conditions(C) and Dependency on activities(D) along with mutability of activities create a complex but reasonable model for smart collaborative systems. Upon a request for an activity, one or more decision components can have the impact on the final decision of the initiation, continuity or revocation of that activity. In Figure \ref{ACAC core models} (a), we show the combinations of the models in a lattice format. We put the base models at the bottom. At next two levels, models are made using two and three models respectively from the immediate lower levels. $\mathrm{ACAC_{ABCD}}$ is the parent model which combines the four models each of which is a combination of three lower level models. In this paper, we focus on the dependency(D) based on the relationship of activities. In our future work, we will have the complete picture for $\mathrm{ACAC_{A}}$,$\mathrm{ACAC_{B}}$,$\mathrm{ACAC_{C}}$, and $\mathrm{ACAC_{D}}$ models.

\begin{figure}[!t]
\centering
\subfigure[]{\includegraphics[width = \columnwidth]{Figures/ACAC_abcd_v3.png}}

\subfigure[]{\includegraphics[width = \columnwidth]{Figures/preDonD_v1.png}}
%\hfill
%\subfloat[(a)]{\includegraphics[width = .9\columnwidth]{Figures/ACAC_abcd_v1.png}}
\vspace{-2mm}
\caption{$\mathrm{ACAC_{ABCD}}$ Core Models.}
\label{ACAC core models}
\end{figure} 

==> Tables/Initial.tex <==
%\clearpage
\begin{table}[!t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\vspace{-2mm}
\caption{Execution time for pre-check with dynamic number of requests and dependent activities.}
\vspace{-2mm}
\scalebox{0.7}{%
\begin{tabular}{*{15}{|p{3.5cm}|p{1cm}|p{1cm}|p{1.9cm}}}
\hline
\textbf{Number of Requests} & \textbf{NDC}& \textbf{NDU} & \textbf{Time (in ms)} \\

\hline
10&20&10&38.84\\

\vspace{-2mm}
20&30&10&53.33
\\

\vspace{-2mm}
30&50&0&101.33
\\

\vspace{-2mm}
40&60&10&110.16
\\

\hline

\end{tabular}}
%}
\label{initial}
\vspace{-3mm}
\end{table}

%\clearpage

==> Tables/Ongoing.tex <==
%\clearpage
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\centering
\caption{Execution time for ongoing check with dynamic number of requests and dependent activities.}
\vspace{-2mm}
\scalebox{0.7}{%
\begin{tabular}{*{15}{|p{3.5cm}|p{1cm}|p{1cm}|p{1.9cm}}}
\hline
\textbf{Number of Requests} & \textbf{NDC}& \textbf{NDU} & \textbf{Time (in ms)} \\

\hline
10&30&10&42.83\\

\vspace{-2mm}
20&60&30&57.64
\\

\vspace{-2mm}
30&80&0&87.24
\\

\vspace{-2mm}
40&90&10&124.30
\\

\hline

\end{tabular}}
%}
\label{ongoing}
\vspace{-2mm}
\end{table}

%\clearpage

==> Tables/Post.tex <==
%\clearpage
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\centering
\caption{Execution time for post-check with dynamic number of requests and dependent activities.}
\vspace{-2mm}
\scalebox{0.7}{%
\begin{tabular}{*{15}{|p{3.5cm}|p{1cm}|p{1cm}|p{1.9cm}}}
\hline
\textbf{Number of Requests} & \textbf{NDC}& \textbf{NDU} & \textbf{Time (in ms)} \\

\hline
10&20&20&15.21\\

\vspace{-2mm}
20&20&20&22.09
\\

\vspace{-2mm}
30&50&10&25.44
\\

\vspace{-2mm}
40&50&30&60.76
\\

\hline

\end{tabular}}
%}
\label{post}

\end{table}

%\clearpage

==> Tables/Set-Table.tex <==
\begin{table}
%\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1}
\caption{Introduction to basic sets and functions used in the definitions and algortihm}
\begin{tabular*}{\linewidth}{l}
\hline
\textbf{Basic Sets} \\
- $S$, $O$, and $OP$ are finite sets of sources, objects, and operations.\\
%- $S$, $O$, $OP$ and $ACT$ are finite sets of sources, objects, operations and activities in the system respectively.\\
- $ACT$ is a finite set of activities that can be performed in the system.\\
- $ACT_R$ is a set of requested activities where $ACT_R$ = $ACT$.\\
- $ACT_D$ is a set of dependent activities where $ACT_D$ = $ACT$.\\
- $ACT_{DoD}$ is a set of dependent of dependent activities where $ACT_{DoD}$ = $ACT$\\
- $ST$ is a finite set of states of activities and is defined as \{inactive, dormant, aborted, running, revoked, finished\}\\
- $ST_{CR}$ is finite set of current states where $ST_{CR}$ = $ST$.\\
- $ST_{DR}$ is finite set of desired states where $ST_{DR}$ = $ST$.\\
\textbf{Basic Functions}\\
- $getObject: ACT_R \longrightarrow O$, 
 mapping a requested activity to the most suitable object provided by the system.\\\\
 - $getOperation: ACT_R \times O \longrightarrow OP$, mapping a corresponding operation to start the requested activity an object\\\\
 - $getDA: ACT_R \times O \longrightarrow 2^{ACT_D}$, mapping the combination of requested activity and a corresponding object to a\\ \;\; set of dependent activities.\\\\
 - $getCurrentSt: ACT \longrightarrow ST_{CR}$, mapping each activity to a current state.\\\\
 - $getDesiredPreDASt: ACT_R \times O \times ACT_D \longrightarrow 2^{ST_{DR}}$, mapping the combination of a requested activity, an object\\
 \;\; which is suitable to execute the requested activity,
 and a pre dependent activity of the requested activity to a set of\\
 \;\; desired states, one state of which is required for the dependent activity before the requested activity is allowed. \\\\

- $getDesiredOnDASt: ACT_R \times O \times ACT_D \longrightarrow 2^{ST_{DR}}$, mapping the combination of a requested activity, an object\\
 \;\; in which the requested activity is running,
 and an ongoing dependent activity of the requested activity to a set of\\
 \;\; desired states, one state of which is required for the dependent activity during the execution of the requested activity. \\\\
 
 - $getDesiredPostDASt: ACT_R \times O \times ACT_D \longrightarrow 2^{ST_{DR}}$, mapping the combination of a requested activity, an object\\
 \;\; in which the requested activity runs,
 and a post dependent activity of the requested activity to a set of\\
 \;\; desired states, one state of which is required for the dependent activity after the requested activity is performed. \\\\

 - $getDoDA: ACT_D \times ST_{CR} \times ST_{DR} \longrightarrow 2^{ACT_{DoD}}$, mapping the combination of a dependent activity, the current state\\
 \;\; of the dependent activity and a desired state of the dependent activity to a set of dependent of dependent activities.\\\\

 - $getDesiredDoDASt: ACT_D \times ST_{CR} \times ST_{DR} \times ACT_{DoD} \longrightarrow 2^{ST_{DR}}$, mapping the combination of a dependent activity,\\
 \;\; the current state of the dependent activity, desired state of the dependent activity, and a dependent of dependent\\
 \;\; activity to a set of desired states, one of which is required for the dependent of dependent activities to update the\\ \;\; dependent activity from the current state to the desired state.\\
 



\hline
\end{tabular*}
\end{table}

==> Tables/Table1_Model_Space.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.5}
\centering

\caption{$\mathrm{ACAC_{D}}$ Models}
\vspace{-2mm}
%\hl{Table I is modified and ready to review}
%\rowcolors{1}{lightgray!20!}{}
\scalebox{1}{%
\begin{tabular}{*{15}{|p{3cm}|p{3cm}|p{3cm}|p{3cm}}}

\hline
 & \textbf{Immutable (0)} & \textbf{Pre-update (1)}& \textbf{Ongoing-update (2)} & \textbf{Post-update (3)} \\
\hline

preD&Y&Y&N&Y\\
\vspace{-2mm}
onD&Y&N&Y&Y

 \\
\hline

\end{tabular}

}
%\label{tabax}
\label{model space}
\end{table*}

==> Tables/Table2_CharacterizationsAndModels.tex <==
%\clearpage
\begin{table}[!t]
\centering
\caption{}
\vspace{-2mm}
\rowcolors{1}{lightgray!20!}{}
\scalebox{0.9}{%
\begin{tabular}{*{10}{p{1.4cm}}}
\hline

\textbf{Activities Relationship} &  \textbf{$preD_0$}& \textbf{$preD_1$} & \textbf{$preD_3$} &
\textbf{$onD_0$} &
\textbf{$onD_1$} &
\textbf{$onD_2$} &
\textbf{$onD_3$} \\
\hline
Ordered & \;\;\;\;\; $\times$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\times$& \;\;\;\;\; $\surd$& \;\;\;\;\; $\times$&
\;\;\;\;\; $\surd$
 \\
\hline
Concurrent  & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\surd$& \;\;\;\;\; $\times$& \;\;\;\;\; $\surd$&
\;\;\;\;\; $\times$
\\
\hline
Temporary & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\;  $\times$ & \;\;\;\;\; $\times$& \;\;\;\;\; $\times$& \;\;\;\;\; $\times$ &\;\;\;\;\; $\times$
 \\
 \hline
Precedence &\;\;\;\;\; $\times$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\times$& \;\;\;\;\; $\surd$& \;\;\;\;\; $\surd$&
\;\;\;\;\; $\surd$
 \\
  \hline
Dependence &\;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$& \;\;\;\;\; $\surd$& \;\;\;\;\; $\surd$&
\;\;\;\;\; $\surd$
 \\
 \hline
Conditional &\;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\times$ &
\;\;\;\;\; $\times$
 \\
 \hline
Incompatible &\;\;\;\;\; $\times$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\times$ & \;\;\;\;\; $\surd$ & \;\;\;\;\; $\surd$ &
\;\;\;\;\; $\surd$
 \\
\hline

\end{tabular}}
%}
\label{tab6:mutability}

\end{table}

%\clearpage

==> Tables/requests.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.5}
\centering

\caption{Description of activity requests and dependencies}
\vspace{-2mm}
%\hl{Table I is modified and ready to review}
%\rowcolors{1}{lightgray!20!}{}
\scalebox{0.8}{%
\begin{tabular}{*{15}{|p{2.7cm}|p{4.5cm}|p{4.2cm}|p{3.6cm}}}
\hline

\textbf{Requests} & \textbf{Pre-dependent activities}&\textbf{Ongoing-dependent activities}& \textbf{Post-dependent activities}\\
\hline
\textit{request(fieldWorker,
sprayingWeedKiller)}&
\vspace{-1.5mm}
 \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{weedScanning} : \textit{running}
  \item \textit{moistureMonitoring} : \textit{running}
\end{itemize}
\vspace{-2mm}&
\vspace{-1.5mm}
 \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{weedScanning} : \textit{running}
  \item \textit{thermalImaging} : running
  \item \textit{nitrogenMonitoring} : \textit{running}
\vspace{-1.7mm}
\end{itemize}
\vspace{-1.5mm}&
\vspace{-1.5mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{waterSpray} : \textit{running}
  \item \textit{weedScanning} : \textit{inactive}
  \vspace{-1.5mm}
\end{itemize}
\\
\rowcolor{lightgray!40!}
\hline
\textit{request(farmer, sowingSeeds)}&
\vspace{-1.5mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{fieldPloughing} : \textit{inactive}
\end{itemize}&
\vspace{-0.7mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
\vspace{-1.5mm}
  \item \textit{pesticideSpray} : \textit{running}
  \item \textit{thermalImaging} : \textit{running}
  \item \textit{airCooling} : \textit{running}
\vspace{-1.7mm}
\end{itemize}
\vspace{-1.5mm}&
N/A
 \\
 \hline
\textit{request(farmManager, fieldPloughing)}&
 \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
\vspace{-1.5mm}
  \item \textit{proximityMeasureToGroundWater} : \textit{running}
  \item\textit{surfaceTemperatureMeasurement} : \textit{running}
  \vspace{-1.9mm}
\end{itemize}&
\vspace{-1.7mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{waterSpray} : \textit{running}
  \item \textit{thermalImaging} : \textit{running}
  \vspace{-1.5mm}
\end{itemize}&
\vspace{-1.5mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{weedKillerSpray} : \textit{running}
  \item \textit{sowingSeeds} : \textit{running}
  \item \textit{pesticideSpray} : \textit{running}
  \vspace{-1.7mm}
\end{itemize}
 \\
  \rowcolor{lightgray!40!}
 \hline
\textit{request(fieldOwner, coolingGreenhouse)}&
\vspace{-0.7mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
\vspace{-1.7mm}
  \item \textit{thermalImaging} : \textit{running}
\end{itemize}&
\vspace{-2mm} \begin{itemize}[noitemsep,nolistsep,leftmargin=*]
  \item \textit{humidifying} : \textit{running}
\end{itemize}&N/A
 \\
\hline
%\hline

\end{tabular}

}
\label{request}
\vspace{-4mm}
\end{table}

%\vspace{-2mm}
